Defining and comparing SICR-events for classifying impaired loans under IFRS 9

The IFRS 9 accounting standard requires the prediction of credit deterioration in financial instruments, i.e., significant increases in credit risk (SICR). However, the definition of such a SICR-event is inherently ambiguous, given its current reliance on evaluating the change in the estimated probability of default (PD) against some arbitrary threshold. We examine the shortcomings of this PD-comparison approach and propose an alternative framework for generating SICR-definitions based on three parameters: delinquency, stickiness, and the outcome period. Having varied these framework parameters, we obtain 27 unique SICR-definitions and fit logistic regression models accordingly using rich South African mortgage and macroeconomic data. For each definition and corresponding model, the resulting SICR-rates are analysed at the portfolio-level on their stability over time and their responsiveness to economic downturns. At the account-level, we compare both the accuracy and dynamicity of the SICR-predictions, and discover several interesting trends and trade-offs. These results can help any bank with appropriately setting the three framework parameters in defining SICR-events for prediction purposes. We demonstrate this process by comparing the best-performing SICR-model to the PD-comparison approach, and show the latter's inferiority as an early-warning system. Our work can therefore guide the formulation, modelling, and testing of any SICR-definition, thereby promoting the timeous recognition of credit losses; the main imperative of IFRS 9.

==> old-4.2-OutcomePeriodEffect.tex <==
\subsection{The effect of the outcome period \texorpdfstring{$k$}{Lg} when defining and predicting SICR-events}
\label{sec:outcomePeriods}


In general, SICR-classification should react dynamically to changes in credit risk and its pre-default evolution over time. This dynamicity is even implicit in \S B5.5.2 of IFRS 9, which postulates that a SICR-event should ideally predate an increase in loan delinquency, i.e., the $g_0$-measure. In predicting such events, shorter outcome periods $k$ can demonstrably achieve this dynamicity more readily than longer periods, since the latter is at greater risk of missing short-term fluctuations in $g_0(t)$ between times $t$ and $t+k$. However, the `optimal' choice of this outcome period is yet unclear, as is the very idea of optimality within this SICR-modelling context. 
% Explain and defend setup
To help fill this gap, we deliberately vary $k$ from 3 months up to an extreme of 36 months when training our (cross-sectional) SICR-models, at least within this particular subsection. 
% Rebut use of a lifetime measure
The resulting $k$-month forward SICR-predictions, as rendered over loan life, can reasonably approximate their true lifetime counterpart, especially so for smaller $k$-values. This approximation is reminiscent of using a series of risk estimates from a 12-month PD-model (see appendix) in approximating a lifetime PD-measure, as permitted in \S B5.5.13 of IFRS 9.
However, future work can certainly extend our cross-sectional approach to a more dynamic one, e.g., by using survival analysis. Doing so can enable SICR-prediction across any number of $k$-values over loan life, instead of just the 7 fixed $k$-values that we currently explore in first establishing some factual basis.


% Experimental setup: other considerations
Aside from the $k$-parameter, the other parameters of the SICR-framework are kept constant at $d=1$ and $s=1$ for this experiment, which resolves to definition class 1a within \autoref{tab:SICR_Defs}. These two values are relatively benign for the following two reasons. 
Firstly, the underlying SICR-test $g_0(t)\geq d$ from \autoref{eq:bool_decision} suggests that $d=2$ will yield a subset of SICR-outcomes that are already selected by $d=1$. The latter choice of $d=1$ therefore leads to a `broader' SICR-definition that already encompasses the SICR-outcomes that are specifically isolated by the more `narrow' $d=2$ definition class. 
Secondly, $s=1$ implies zero `stickiness' and simplifies the resulting SICR-definition. Both choices of $d$ and $s$ should therefore have minimal interference when studying the effect of $k$, as intended in this experiment.

\begin{figure}[ht!]
\centering\includegraphics[width=0.78\linewidth,height=0.71\textheight]{TimeGraph_SICR-Incidence_Actual_1a.png}
\caption{Comparing actual SICR-rates over time and across outcome periods $k\in\{3,6,9,12,18,24,36\}$ within $\mathcal{D}_S$ for SICR-definition class 1a from \autoref{tab:SICR_Defs}. The mean and standard deviation of each resulting time series are summarised within the inset graphs. Encircled points denote the maximum of each series over time.}\label{fig:1a_SICR_Rates_Actual}
\end{figure}


% SICR-rates
As a first step, it is useful to explore the portfolio-level effect of a given SICR-definition by using the \textit{SICR-rate}, as defined in the appendix.
The observed SICR-rates are shown in \autoref{fig:1a_SICR_Rates_Actual} over time and across all chosen $k$-values. Evidently, each time graph has a different but increasing mean-level as $k$ increases, especially when examined after the anomalous 2008 Global Financial Crisis (GFC). However, a longer outcome period invariably allows greater opportunity for a Stage 1 account to develop sufficient delinquency; enough to enter -- and remain in -- default. Since $g_0(t+k)\geq 3 > d$ from \autoref{eq:bool_decision} will hold for both default and SICR-outcomes respectively, larger $k$-values will therefore increasingly capture a greater proportion of defaulting accounts. This phenomenon explains the increasing mean SICR-rates that are correlated with increasing $k$-values; a relationship that becomes almost linear when removing the 2008-GFC period during the calculation of the SICR-mean. In fact, \autoref{fig:1a_SICR_Rates_Actual} shows that overall mean-levels seemingly reach a plateau near $4\%$ for $k\geq 12$, having rapidly increased for smaller $k$-values. At the very least, this may suggest that choosing $k\geq18$ has a negligible contribution to the overall SICR-mean, which may already have stabilised at $k=12$. At worst, choosing $k\geq 18$ will increasingly select default-instances into the sample, thereby `contaminating' the SICR-mean. Doing so can detract from the very idea of SICR-staging, which should ideally act as a pro-cyclical early warning system for impending credit risk; see \S B.5.5.21 in IFRS 9 from \citet{ifrs9_2014} and \citet{gaffney2019cyclicality}.


Apart from differing SICR-means, \autoref{fig:1a_SICR_Rates_Actual} shows that each $k$-value results in a time graph with a different volatility pattern. Evidently, the SICR-rates of extreme $k$-values are more stable over time relative to other $k$-values. In particular, the series resulting from $k\leq 3$ and $k > 24$ exhibit lower standard deviation than their peers. However, stable SICR-rates may not necessarily be a useful pursuit, especially not during an unfolding macroeconomic crisis and its subsequent effect on default rates. While the SICR-rates associated with extreme $k$-values are relatively stable, they also failed to track the increasing default rates during the volatile 2008-GFC period. As a working principle, and when defining SICR-events, the resulting SICR-rates should reasonably exceed default rates (or some lagged variant thereof) since SICR-staging should ideally preempt default. 
This principle avails a useful heuristic in disqualifying both $k\leq 3$ and $k>24$, given the 12-month default rate of about $6\%$ that prevailed at the height of the 2008-GFC; see the appendix. 


\begin{figure}[ht!]
\centering\includegraphics[width=0.62\linewidth,height=0.4\textheight]{Summaries_SICR-Incidence_Actual_1a.png}
\caption{Various summary statistics of the actual SICR-rates from \autoref{fig:1a_SICR_Rates_Actual} across chosen outcome periods $k$ for SICR-definition class 1a from \autoref{tab:SICR_Defs}. Summaries include the earliest, maximum, and mean after Dec-2009 (`post-GFC'), as well as differences amongst these summaries, i.e., the early-warning degree and the post-GFC recovery degree. Desirable $k$-values are encircled and discussed.}\label{fig:1a_SICR_Rates_Actual-Summary}
\end{figure}


For each of the remaining $k$-values, the earliest SICR-rate $a(k)$ (at January-2007) can be compared to the maximum SICR-rate $b(k)$, which typically occurs during the 2008-GFC. Effectively, this comparison constitutes the degree to which a SICR-definition can respond to unfolding calamities. The \textit{early-warning degree} $b(k)-a(k)$ is graphed in \autoref{fig:1a_SICR_Rates_Actual-Summary} in pink; larger values are deemed as better. Clearly, $k\in[6,12]$ yield SICR-rates that reassuringly increased by about 2\%-3\% points from January-2007 leading into the crisis, thereby demonstrating considerable responsiveness to externalities like the 2008-GFC. 
Furthermore, the maxima $b(k)$ can be compared to the post-crisis SICR-means $c(k)$ in measuring the magnitude by which the resulting SICR-rate can normalise. The \textit{recovery degree} $b(k)-c(k)$ is shown in \autoref{fig:1a_SICR_Rates_Actual-Summary} in green; larger values are again deemed as better. The SICR-rates resulting from $k\in[6,12]$ recovered substantially by about 5\%-7\% points back to their post-GFC SICR-means, which suggests appropriate resiliency within the underlying definitions. While $k\in[18,24]$ had similar recovery degrees, the resulting SICR-rates are already high even before the 2008-GFC. Accordingly, longer outcome periods cannot timeously signal impending distress and would likely result in SICR-models that produce predictions that are overly conservative and even financially punitive; i.e., `paranoid'.
In the extreme case, very long outcome periods such as $k\geq 36$ can miss the entirety of a crisis period, as evidenced by low-values for both the early-warning and post-GFC recovery degrees. In contrast, SICR-definitions with shorter outcome periods $k\leq 12$ can react more flexibly during market failures without becoming punitive ahead of time; a desirable quality.


% AUC-results
In assessing the SICR-model that results from each SICR-definition, a few performance measures are formulated in the appendix and subsequently calculated and summarised in \autoref{tab:1a-performance}.
Firstly, the prediction accuracy of each logit-model is evaluated by estimating the \textit{receiver operating characteristics} (ROC) graph from the predictions within the validation set $\mathcal{D}_V$. The interested reader is referred to \citet{fawcett2006introduction} regarding ROC-analyses, which are typically summarised into a single statistic called the \textit{area under the curve} (AUC). Equipped with such AUC-values, the results in \autoref{fig:1a-AUC_a} suggest that smaller outcome periods yield more accurate SICR-models than longer periods. This trend is also reflected in the widening confidence intervals of these AUC-values as $k$ increases. Reassuringly, this finding corroborates the work of \citet{kennedy2013window} and \citet{mushava2018experimental} wherein the outcome period was similarly varied in PD-modelling -- an older `cousin' of SICR-modelling -- which resulted in a similar AUC-trend across $k$-values. Moreover, the nonlinear reduction in successive AUC-values seems to subside after $k\geq24$, which suggests yet again that examining smaller $k\leq 18$ values is a more worthwhile endeavour. 
Having dichotomised the SICR-predictions using fixed $c_{dsk}$-thresholds, the resulting AUC-values follow a similar (though even more pronounced) downwards trend as $k$ increases; see \autoref{fig:1a-AUC_b}.  
Longer outcome periods also result in fewer observed SICR-outcomes, as evidenced by a decreasing prevalence rate $\phi_{dsk}$. Since the Generalised Youden Index $J_a$ contains this $\phi_{dsk}$-quantity (see appendix), a rarer SICR-outcome therefore explains why the cut-off $c_{dsk}$ decreases in tandem with greater $k$-values. More generally, fewer SICR-outcomes can exacerbate the task of finding a statistical relationship using logistic regression, hence why the AUC decreases as $k$ increases.


\begin{table}[ht!]
\caption{Various performance measures for evaluating SICR-models across different $k$-values within definition class 1a ($d=1,s=1$) from \autoref{tab:SICR_Defs}. AUC-values are given with 95\% confidence intervals (DeLong-method) for both probabilistic and discrete SICR-classifiers, as applied on $\mathcal{D}_V$. The prevalence, dynamicity, and instability measures are calculated within $\mathcal{D}_S$; see the appendix for their definitions.}
\label{tab:1a-performance}
\centering
\begin{tabular}{p{1.35cm} p{1.4cm} p{1.5cm} p{2.1cm} p{1.6cm} p{1.4cm} p{1.2cm} p{2.1cm}}
\toprule
\textbf{Definition} & \textbf{Outcome period} $k$ & \textbf{Prevalence} $\phi_{dsk}$ & \textbf{AUC-Probabilistic} & \textbf{Dynamicity} $\omega_{dsk}$ & \textbf{Instability} $\sigma_{dsk}$ & \textbf{Cut-off} $c_{dsk}$ & \textbf{AUC-Discrete}  \\ \midrule
\rowcolor[HTML]{ECF4FF} 
1a(i) & $k=3$ & 6.16\% & 91.3\% \footnotesize{$\pm$ 0.48\%} & 4.3\% & 1.00\% & 12.0\% & 82.4\% \footnotesize{$\pm$ 0.66\%}  \\
\rowcolor[HTML]{ECF4FF} 
1a(ii) & $k=6$ & 6.13\% & 88.5\% \footnotesize{$\pm$ 0.54\%} & 3.8\% & 1.43\% & 10.9\% & 78.1\% \footnotesize{$\pm$ 0.70\%} \\
\rowcolor[HTML]{ECF4FF} 
1a(iii) & $k=9$ & 6.07\% & 86.5\% \footnotesize{$\pm$ 0.57\%} & 3.6\% & 1.64\% & 11.5\% & 74.9\% \footnotesize{$\pm$ 0.73\%} \\
\rowcolor[HTML]{ECF4FF} 
1a(iv) & $k=12$ & 5.99\% & 84.8\% \footnotesize{$\pm$ 0.60\%} & 3.4\% & 1.81\% & 11.6\% & 73.4\% \footnotesize{$\pm$ 0.72\%} \\
\rowcolor[HTML]{ECF4FF} 
1a(v) & $k=18$ & 5.73\% & 82.2\% \footnotesize{$\pm$ 0.67\%} & 2.8\% & 1.60\% & 11.3\% & 70.9\% \footnotesize{$\pm$ 0.74\%} \\
\rowcolor[HTML]{ECF4FF} 
1a(vi) & $k=24$ & 5.46\% & 80.6\% \footnotesize{$\pm$ 0.71\%} & 2.5\% & 1.27\% & 11.3\% & 68.7\% \footnotesize{$\pm$ 0.76\%} \\
\rowcolor[HTML]{ECF4FF} 
1a(vii) & $k=36$ & 5.19\% & 79.0\% \footnotesize{$\pm$ 0.76\%} & 2.0\% & 0.65\% & 9.8\% & 67.9\% \footnotesize{$\pm$ 0.78\%} \\ \bottomrule
\end{tabular}
\end{table}


\begin{figure}[ht!]
\centering
\begin{subfigure}{0.49\textwidth}
    \caption{Logistic Regression (Probabilistic)}
    \centering\includegraphics[width=1\linewidth,height=0.34\textheight]{"ROC_1a_logit_prob_k-values".png}\label{fig:1a-AUC_a}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
    \caption{Logistic Regression (Discrete)}
    \centering\includegraphics[width=1\linewidth,height=0.34\textheight]{"ROC_1a_logit_disc_k-values".png}\label{fig:1a-AUC_b}
\end{subfigure}
\caption{ROC-analysis of the SICR-predictions in $\mathcal{D}_V$ resulting from SICR-models developed with definition class 1a ($d=1,s=1$) from \autoref{tab:SICR_Defs}, having varied the outcome period $k$. In \textbf{(a)}, the probability scores from each SICR-model are evaluated as predictions. In \textbf{(b)}, the same scores are dichotomised into discrete predictions using the corresponding cut-off $c_{dsk}$ from \autoref{tab:1a-performance}. The AUC-values are printed, together with 95\% confidence intervals (DeLong-method) and corresponding Gini-values.}\label{fig:1a-AUC}
\end{figure}


% Prediction dynamicity
Pursuing greater AUC-values may at first seem worthwhile when selecting a SICR-definition; however, there are other considerations. In particular, one can measure the degree to which a SICR-model's predictions vary over the lifetime of an average account, i.e., the prediction dynamicity $\omega_{dsk}$, as provided in \autoref{tab:1a-performance}. 
Evidently, SICR-models built from shorter outcome periods yield predictions that vary more over time $t$, relative to longer outcome periods. Like the AUC-values, $\omega_{dsk}$ appears to be a monotonically decreasing function of $k$, which invariably couples greater accuracy with greater dynamicity (or variance) as a necessary consequence. 
Considering the portfolio-level SICR-rates in \autoref{fig:1a_SICR_Rates_Actual}, it is also clear that the underlying SICR-process is itself dynamic and stochastic over time upon its aggregation to the portfolio-level, albeit to different extents given $k$. Moreover, and barring the extremes ($k\leq 3$), \autoref{fig:1a_SICR_Rates_Actual-Summary} shows that shorter outcome periods also yield more responsive SICR-rates leading up to the 2008-GFC, despite the more volatile SICR-predictions at the account-level. 
Lastly, this relationship between accuracy and variance is reminiscent of a well-known phenomenon within all statistical learning, called the \textit{bias-variance trade-off}; see \citet[\S 2.9,~\S 7]{hastie2009elements} and \citet[\S 2]{james2013introduction}.



On the other hand, the dynamicity in account-level SICR-predictions, as measured by $\omega_{dsk}$ when varying $k$, may not necessarily produce the same dynamicity at the portfolio-level. 
It is true that SICR-outcomes defined using extremely short outcome periods $k\leq 3$ can demonstrably lead to highly dynamic (and accurate) SICR-predictions at the account-level. However, the same volatile SICR-predictions stabilise somewhat upon their aggregation into the portfolio-level expected SICR-rate. 
It is therefore useful to compare the account-level $\omega_{dsk}$-measure against its portfolio-level counterpart, i.e., the \textit{instability} $\sigma_{dsk}$, as defined in the appendix, summarised in \autoref{tab:1a-performance}, and shown in the inset graph of \autoref{fig:1a_SICR_Rates_Actual}. Evidently, extremely dynamic SICR-predictions, as produced with $k\leq 3$, can lead to rapid oscillations in moving an account between Stages 1 and 2 over time. This oscillatory effect dampens the overall transition into Stage 2 when aggregating across accounts, hence the less responsive SICR-rate in \autoref{fig:1a_SICR_Rates_Actual-Summary} (in pink) and the lower $\sigma_{dsk}$-values when selecting $k\leq 3$. It is therefore questionable to adopt such extremely short outcome periods when, despite their greater prediction accuracy, the associated volatility of the resulting SICR-predictions do not meaningfully translate into more dynamic SICR-rates, as expected at the portfolio-level.


Having disqualified $k\leq 3$, we can similarly disregard $k\geq 18$ given the worsening accuracy (AUC) of the associated SICR-predictions. Larger $k$-values also result in less dynamic SICR-predictions over time, as is evident in the decreasing $\omega_{dsk}$-values. Simultaneously, the resulting SICR-rates from these larger $k$-values are seemingly less responsive to externalities such as the 2008-GFC, given the decreasing early-warning degree. Regarding the remaining $k$-choices, we note that the rate of change in $\omega_{dsk}$ from \autoref{tab:1a-performance} slows down significantly for $k\in[6,12]$. This plateauing effect suggests that selecting slightly larger $k$-values within this range will not overly erode the dynamicity of account-level SICR-predictions. At the same time, the progressively larger $\sigma_{dsk}$-values, as associated with $k\in \{6,9, 12\}$, imply that those SICR-rates are more dynamic, especially in response to an unfolding macroeconomic crisis. The midpoint hereof is $k=9$, which seems `optimal' when considering the trade-offs amongst: 1) the AUC-values; 2) $\omega_{dsk}$; 3) $\sigma_{dsk}$; and 4) the early-warning and recovery degrees in measuring the crisis responsiveness.


\begin{figure}[ht!]
\centering
\begin{subfigure}{0.49\textwidth}
    \caption{1a(i): $k=3$}
    \centering\includegraphics[width=1\linewidth,height=0.28\textheight]{"TimeGraph_SICR-Incidence_ActExp1a-i".png}\label{fig:1a_SICR_Rates_a}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
    \caption{1a(ii): $k=6$}
    \centering\includegraphics[width=1\linewidth,height=0.28\textheight]{"TimeGraph_SICR-Incidence_ActExp1a-ii".png}\label{fig:1a_SICR_Rates_b}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
    \caption{1a(iii): $k=9$}
    \centering\includegraphics[width=1\linewidth,height=0.28\textheight]{"TimeGraph_SICR-Incidence_ActExp1a-iii".png}\label{fig:1a_SICR_Rates_c}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
    \caption{1a(iv): $k=12$}
    \centering\includegraphics[width=1\linewidth,height=0.28\textheight]{"TimeGraph_SICR-Incidence_ActExp1a-iv".png}\label{fig:1a_SICR_Rates_d}
\end{subfigure}
\caption{Time graphs of actual versus expected SICR-rates within $\mathcal{D}_S$ for SICR-definition class 1a ($d=1,s=1$) across shorter outcome periods $k\in \{3,6,9,12\}$. In creating the discretised expected rate $C_t$, the SICR-model is first dichotomised by using the corresponding cut-off $c_{dsk}$. The MAEs between the actual and each expected SICR-rate are overlaid in summarising the line graph discrepancies over time.}\label{fig:1a_SICR_Rates}
\end{figure}


% Actual vs expected time graphs
The time graphs of actual versus expected SICR-rates are shown in \autoref{fig:1a_SICR_Rates} for each $k\in\{3,6,9,12\}$, denoted respectively as $A_t$ and $B_t$ over calendar time $t$, and calculated as described in the appendix. Ideally, both time graphs (green and orange) should closely overlap each other, thereby implying that the aggregated predictions agree with reality, which also indicates an excellent SICR-model. One can measure the level of such agreement by calculating the \textit{mean absolute error} (MAE) between $A_t$ and $B_t$ over $t$, where this MAE is denoted by $m_1$ and printed in \autoref{fig:1a_SICR_Rates} for some $k$-values.
% MAE-values
Barring the extreme case of $k\geq 36$, all $m_1$-values are fairly similar with a mean error of 0.44\% across $k$, which is reassuringly low and corroborates the relatively high AUC-values in \autoref{tab:1a-performance}. Evidently, the underlying SICR-models can accurately predict SICR-outcomes regardless of $k$, despite the aggregated SICR-rates becoming less responsive to externalities as $k$ increases. 


% Actual vs expected (discrete) time graphs
A \textit{discretised} expected SICR-rate emerges in \autoref{fig:1a_SICR_Rates} when first dichotomising the SICR-models using $c_{dsk}$ before calculating the SICR-rate, as described in the appendix. The resulting rate $C_t$ (purple) is similarly compared to $A_t$ by calculating the associated MAE; itself denoted as $m_2$ and printed in \autoref{fig:1a_SICR_Rates}. Clearly, there are some large discrepancies between $A_t$ and $C_t$ during some periods, particularly during the 2008-GFC, with a mean $m_2$-value of 1.11\% across $k\in\{3,6,9,12,18,24,36\}$; almost three times larger than the mean $m_1$-value. Nonetheless, the smallest $m_2$-value occurred at $k=9$, which further supports its choice as the `optimal' outcome period. Experimentation showed however that $C_t$ is highly sensitive to the choice of the $c_{dsk}$-value, which can certainly be tweaked in future work. In this regard, when estimating the associated Generalised Youden Index $J_a$, the misclassification cost ratio $a$ can be further increased in minimising false negatives. Doing so should at least increase the prevalence of $C_t\geq A_t$ over $t$, i.e., rather the bank be over-provided than under-provided in its loss provision; a risk-prudent outcome under IFRS 9. Moreover, the $a$-value can itself be attuned to a chosen SICR-definition and the resulting SICR-model, instead of fixing $a$ to a single value across all SICR-definitions, as in this study. 


==> old-6.2-LogisticRegression.tex <==
\subsection{Logistic regression as supervised classifier technique}
\label{app:logistic}

Like many supervised techniques, logistic regression aims to find a statistical relationship between a set of random input variables $\boldsymbol{X}$ and the binary-valued outcome (or Bernoulli random variable) $Y\in\left\{\mathcal{C}_0:0 \ ; \ \mathcal{C}_1:1\right\}$. This $Y$ records either a non-event $\left(\mathcal{C}_0\right)$ or a SICR-event $\left(\mathcal{C}_1\right)$, both of which are also called a `negative' or `positive' respectively. From \citet[pp.~1--10]{hosmer2000logistic}, \citet[\S4]{bishop2006pattern}, \citet[\S4]{hastie2009elements}, and \citet[\S4.3]{james2013introduction}, the focus of logistic regression is on estimating the conditional mean $\mathbb{E}\left[Y \vert \boldsymbol{X} \right]$ as the probability of class $Y$ given $\boldsymbol{X}$. 
Let $p_1(\boldsymbol{x})\in \left[0,1\right]$ be an estimate of the posterior class probability of $Y=\mathcal{C}_1$ given the realisation $\boldsymbol{x}$ from a $p$-dimensional random vector $\boldsymbol{X}$. The conditional mean $\mathbb{E}\left[Y \vert \boldsymbol{X} \right]$ is commonly modelled using the standard logistic function $\sigma: \mathbb{R} \rightarrow [0,1]$, itself defined as $\sigma(w)= e^w / (1+e^w)= (1+e^{-w})^{-1}$. Then, $w$ is replaced with a linear combination $\boldsymbol{\beta}^T\boldsymbol{x}$ of the realised input variables $\boldsymbol{x}=\left\{x_1,\dots,x_p\right\}$ and its associated coefficient vector $\boldsymbol{\beta}=\left\{\beta_1,\dots,\beta_p\right\}$ with intercept $\beta_0$. Accordingly, $\mathbb{E}\left[Y \vert \boldsymbol{X} \right]$ is expressed respectively for either class $\mathcal{C}_1$ or $\mathcal{C}_0$ as \begin{align} \label{eq:logistic}
    \mathbb{P}\left[Y=\mathcal{C}_1 \vert \boldsymbol{X} = \boldsymbol{x} \right] &&\approx&& p_1(\boldsymbol{x}) &&=&&& \frac{\exp\left(\boldsymbol{\beta}^T\boldsymbol{x}+\beta_0\right)}{1 + \exp\left(\boldsymbol{\beta}^T\boldsymbol{x}+\beta_0\right) } &&=&&&& \big(1+e^{-\boldsymbol{w}} \big)^{-1}  \quad \text{and} &&{} \nonumber \\
    \mathbb{P}\left[Y=\mathcal{C}_0 \vert \boldsymbol{X} = \boldsymbol{x} \right] &&\approx&& 1- p_1(\boldsymbol{x}) &&=&&& \frac{1}{1 + \exp\left(\boldsymbol{\beta}^T\boldsymbol{x}+\beta_0\right)} &&=&&&& \big(1+e^{\boldsymbol{w}} \big)^{-1} \, . &&{}    
\end{align} 

Dividing $p_1(\boldsymbol{x})$ in \autoref{eq:logistic} by $1-p_1(\boldsymbol{x})$ yields the \textit{odds} in favour of class $\mathcal{C}_1$ occurring. Taking the natural log hereof then transforms the odds into a (more appealing) symmetric quantity. E.g., the natural log of an odds (in favour) of 4:1 versus its opposite of 1:4 is 0.602 and -0.602 respectively. More formally, the function $g(\boldsymbol{x})=\ln{\left[ \frac{p_1(\boldsymbol{x})}{1-p_1(\boldsymbol{x})} \right]}$ effectively maps the linear combination $\boldsymbol{\beta}^T\boldsymbol{x}+\beta_0$ to the \textit{log-odds} or \textit{logit}, which is the inverse of the logistic function; i.e., $p_1(\boldsymbol{x}) = \sigma\big( g(\boldsymbol{x}) \big)$. 
The logit $g(\boldsymbol{x})$ avails many of the desirable properties of a linear regression model, e.g., the output of $g(\boldsymbol{x})$ may be continuous, can range from $-\infty$ to $\infty$, and is linear in its parameters. Lastly, the unknown regression coefficients $\boldsymbol{\beta}$ in \autoref{eq:logistic} are found using the classical \textit{maximum likelihood estimation} procedure from statistical literature. That is, $\boldsymbol{\beta}$-values are found such that the predicted probability $p_1(\boldsymbol{x}_i)$ of each observation $i$ approximates the observed 0/1-encoded $y_i$-value as closely as possible, given a dataset $\mathcal{D}=\left\{y_i, \boldsymbol{x}_i \right\}$ for $i=1,\dots,n$.

For each trained logit-model, the probability scores $p_1(\boldsymbol{x})$ that estimate $\mathbb{P}\left[\mathcal{C}_1 \vert \, \boldsymbol{x} \right]$ will need to be dichotomised (or discretised) in yielding binary 0/1-decisions. This dichotomisation implies choosing a cut-off $c\in [0,1]$ such that the discretised classifier $h(\boldsymbol{x})=1$ if $p_1(\boldsymbol{x}) > c$ and $h(\boldsymbol{x})=0$ if otherwise. For every possible $c$-value, the probability of a true positive (or SICR-event correctly predicted as such) is $q(c)=\mathbb{P}\left(p_1(\boldsymbol{x}) > c \, | \, \mathcal{C}_1\right)$, also known as sensitivity. Likewise, the probability of a true negative (or non-event correctly predicted as such) is $p(c)=\mathbb{P}\left(p_1(\boldsymbol{x}) \leq c \, | \, \mathcal{C}_0\right)$, also called specificity. In finding the optimal cut-off $c^*$ that incorporates both sensitivity and specificity, consider the Youden Index $J$ that is widely used in the biostatistical literature; see \citet{youden1950index}, \citet{greiner2000principles}, and \citet{schisterman2008youden}. This index $J$ is defined as the maximisation problem \begin{equation} \label{Youden_Index}
    J = \max_c{ \left\{q(c) + p(c) -1 \right\} } \, .
\end{equation} 
Clearly, the classical $J$ assigns equal weight to both sensitivity and specificity, which inappropriately equates the misclassification cost of a false negative to that of a false positive. However, the Generalised Youden Index $J_a$ improves upon $J$ by rendering $c$ sensitive to both types of misclassification costs; see \citet{geisser1998comparing}, \citet{kaivanto2008maximization}, and \citet{schisterman2008youden}. In particular, let $a>0$ be a cost multiple (or ratio) of a false negative relative to a false positive. If $\phi$ is the estimated prevalence of the $\mathcal{C}_1$-event, i.e., the prior $\mathbb{P}\left( \mathcal{C}_1 \right)$, then $J_a$ is expressed for a given $c$ as \begin{equation} \label{eq:gen_Youden_Index}
    J_a(c)= q(c) + \frac{1-\phi}{a\phi} \cdot p(c) - 1 \, ,
\end{equation} whereupon $c^*$ is given by \begin{equation} \label{eq:optimalCutoff}
    c^* = \arg \max_c{J_a(c)} \,.
\end{equation}

The use of logistic regression in binary classification is ubiquitous, particularly in the field of application credit scoring, as was first demonstrated in \citet{wiginton1980}. In this regard, logistic regression is considered by many authors to be the most successful regression technique in quantitative finance; see \citet{hand1997statistical}, \citet[\S4.5,~\S10--11]{thomas2002credit}, \citet{siddiqi2005credit}, \citet[\S1]{thomas2009consumer}, and \citet{bolton2010logistic}. Beyond application credit scoring, this technique is also typically used in pre-screening loan offers, detecting fraud cases, scoring collection success, informing direct marketing offers, and in risk-based pricing. As such, the ubiquity of the logistic regression technique suggests its use in the present study. At the very least, this technique and its results can serve as a benchmark when using more advanced classification techniques in future.

==> old-6.3-FeatureSelection.tex <==
\subsection{Feature selection: constructing the input space of each SICR-model}
\label{app:inputSpace}

% Overview of interactive selection process
In finalising the input space of each SICR-model, we largely followed an interactive, multifaceted, and experimentally-driven process by which variables are selected across repeated logistic regressions.
% Sample size effects on feature selection
One notable challenge to feature selection is that of large sample sizes, which are known to affect $p$-values when testing the statistical significance of regression coefficients, as demonstrated in \citet{lin2013LargeSamples}. The $p$-values can easily approach zero as the sample size increases, notwithstanding the greater statistical power availed by such larger sizes. This phenomenon overlaps with the \textit{Hughes principle} from \citet{hughes1968mean}: a model's predictive power will generally increase for every additional input, but decrease again after reaching some inflection point, provided that the sample size stays constant. 
% Caution against automatic selection processes
Notwithstanding, and during our initial modelling attempts, we experimented with both a best subset approach (stepwise regression) and the LASSO shrinkage method in selecting inputs, as discussed in \citet[\S 6]{james2013introduction}. However, the necessary computation times proved to be excessive (especially for the stepwise method) and even unstable, whilst yielding negligible predictive performance and overly small models. 
Moreover, the declaration of \citet{henderson1981building} -- "the data analyst knows more than the computer" -- seems apt, cautioning against the practice of data dredging when automating feature selection, which is inevitably devoid of human expertise.


% Explain notable parts of selection process
Our interactive selection process is guided by expert judgement, model parsimony, statistical significance, macroeconomic theory, and predictive performance on the validation set $\mathcal{D}_V$. The predictive performance is extensively evaluated using classical ROC-analysis, as summarised by the AUC-measure; see \citet{fawcett2006introduction}.  
% Large sample size issue
In addressing the issue of large sample sizes, we model and select variables using a deliberately larger sub-sampled dataset $\mathcal{D}_S$ of 1 million observations, having applied the same resampling scheme from \cref{app:samplingDesign}. Once the selection process is concluded, the resulting input space is retested for statistical significance on a reduced subsampled set $\mathcal{D}_S$ that only contains 250,000 observations, from which the final SICR-model is also estimated.
We affirm that the vast majority of the inputs remain statistically significant across all $k$-values within each SICR-definition class in \autoref{tab:SICR_Defs}, which further reassures our selection (and `standardisation') process as robust. The interested reader can study our R-codebase on GitHub from \citet{botha2024sourcecode}, which details this process and the associated results as comments within the script of each SICR-model.

In \autoref{tab:featuresdescription}, we summarise and briefly describe the final set of input variables per SICR-definition class. 
Given their widespread prevalence, macroeconomic variables (and their lagged variants) have a notable impact on SICR-events irrespective of definition, which supports the forward-looking information requirement of IFRS 9 from \citet{ifrs9_2014}. This impact is generally greater for SICR-definition class 1 ($d=1$) than for class 2 ($d=2$), while the exact set of macroeconomic variables (MVs) depends on the choice of both $d$ and $s$. By implication, some MVs are more pertinent than others in predicting greater arrears-levels ($d=2$), and \textit{vice versa} for predicting smaller arrears-levels ($d=1$). 
Given the floating interest rates within a mortgage portfolio, it is intuitive that a change in the central bank rate (\verb|Repo_Rate|) immediately affects a borrower's affordability and associated SICR-risk; particularly for $d=1$.
Furthermore, we purposefully included both repo rate and inflation growth despite the former's role in controlling the latter, which implies high collinearity. In extreme market conditions, the supposed structural relationship between these two variables can change due to government intervention, such as during the COVID-19 pandemic. Nonetheless, both variables remain statistically significant across most SICR-models, particularly for $d=1$. 
Furthermore, the variable \verb|PD_ratio| signifies the change in the lifetime PD since initial recognition, which ensures compliance with \S5.5.9 of IFRS 9. Our results, however, show that this variable is statistically insignificant across all SICR-definitions, which implies that the broader input space already captures whatever intrinsic information this variable might have in predicting future SICR-events. 
This profound result clearly rebuts the underlying intuition of \S5.5.9 on incorporating the lifetime PD when rendering SICR-flagging decisions. However, this result is also unsurprising since the associated PD-model (see \cref{app:PD_Model}) has an input space that is similar (but smaller) to those of the various SICR-models. Therefore, not only do these SICR-models predict future SICR-events more accurately, but they also do so more parsimoniously than the PD-comparison approach; an idea now corroborated by this result.



\begin{longtable}{p{3.5cm} p{7.8cm} p{1.8cm} p{2.4cm}}
\caption{The selected input variables across the different SICR-models, given SICR-definitions from \autoref{tab:SICR_Defs}.}
\label{tab:featuresdescription} \\
\toprule
\textbf{Variable} & \textbf{Description} & \textbf{Definitions} & \textbf{Theme} \\ 
\midrule
\endfirsthead
\caption[]{(continued)} \\
\toprule
\textbf{Variable} & \textbf{Description} & \textbf{Definitions} & \textbf{Theme} \\ 
\midrule
\endhead
\midrule \multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
\footnotesize{\verb|ArrearsDir_3|} & \footnotesize{The trending direction of the arrears balance over 3 months, obtained qualitatively by comparing the current arrears-level to that of 3 months ago, binned as: 1) increasing; 2) milling; 3) decreasing (reference); and 4) missing.} & 1a, 1b, 1c, 2a, 2b & Delinquency \\
\footnotesize{\verb|BalanceLog|} & \footnotesize{Log-transformed outstanding balance at month-end.} & 1a, 1c, 2a & Account-level \\
\footnotesize{\verb|BalanceToTerm|} & \footnotesize{Outstanding balance divided by the contractual term of the loan.} & 1b & Account-level \\
\footnotesize{\verb|DebtToIncome|} & \footnotesize{Debt-to-Income: Average household debt expressed as a percentage of household income per quarter, interpolated monthly.} & 1a, 1b, 1c, 2a, 2b & Macroeconomic \\
\footnotesize{\verb|DebtToIncome_12|} & \footnotesize{Debt-to-Income: 12-month lagged version of \verb|DebtToIncome|.} & 1a, 1b, 1c, 2a & Macroeconomic \\
\footnotesize{\verb|Employment_Growth|} & \footnotesize{Year-on-year growth rate in the 4-quarter moving average of employment per quarter, interpolated monthly.} & 2b, 2c & Macroeconomic \\
\footnotesize{\verb|g0_Delinq|} & \footnotesize{Delinquency measure: number of payments in arrears; see $g_0$-measure in \citet{botha2021paper1}.} & 1a, 1b, 1c, 2a, 2b, 2c & Delinquency \\
\footnotesize{\verb|Inflation_Growth|}  & \footnotesize{Year-on-year growth rate in inflation index (CPI) per month.} & 1a, 1b, 1c, 2a, 2b & Macroeconomic \\
\footnotesize{\verb|InterestRate_Margin|} & \footnotesize{Margin between an account's nominal interest rate and the current prime lending rate} & 1a, 1b, 1c, 2a & Account-level \\
\footnotesize{\verb|PayMethod|} & \footnotesize{A categorical variable designating different payment methods: 1) debit order (reference); 2) salary; 3) payroll or cash; and 4) missing.} & 1a, 1b, 1c, 2a & Behavioural \\
\footnotesize{\verb|PD_ratio|} & \footnotesize{Ratio between two estimates of default risk at different time points: the current point in time vs initial recognition. Signifies the change in the lifetime PD; see \cref{app:PD_Model}.} & 1a, 1b, 1c, 2a, 2b, 2c & Delinquency \\
\footnotesize{\verb|PerfSpell_Num|} & \footnotesize{Current performing spell number in tracking previous default spells.} & 1a, 1b, 1c, 2a & Delinquency \\
\footnotesize{\verb|Prepaid_Pc|} & \footnotesize{The prepaid or undrawn fraction of the available credit limit.} & 1a, 1b, 1c, 2a, 2b & Behavioural \\
\footnotesize{\verb|RealGDP_Growth|} & \footnotesize{Year-on-year growth rate in the 4-quarter moving average of real GDP per quarter, interpolated monthly.} & 1a & Macroeconomic \\
\footnotesize{\verb|RealIncome_Growth|} & \footnotesize{Year-on-year growth rate in the 4-quarter moving average of real income per quarter, interpolated monthly.} & 1b, 1c & Macroeconomic \\
\footnotesize{\verb|RealIncome_Growth|} & \footnotesize{12-month lagged version of \verb|RealIncome_Growth|.} & 1b, 1c, 2c & Macroeconomic \\
\footnotesize{\verb|Repo_Rate|} & \footnotesize{Prevailing repurchase rate set by the South African Reserve Bank.} & 1a, 1b, 1c, 2a & Macroeconomic \\
\footnotesize{\verb|RollEver_24|} & \footnotesize{Number of times that loan delinquency increased during the last 24 months, excluding the current time point.} & 1a, 1b, 1c, 2a, 2b, 2c & Delinquency \\
\footnotesize{\verb|Term|} & \footnotesize{Contractual term of the loan.} & 1a, 1b, 1c & Account-level \\
\footnotesize{\verb|TimeInPerfSpell|} & \footnotesize{Duration (in months) of current performing spell before default or competing risk.} & 1a, 1b, 1c, 2a & Delinquency \\ 
\end{longtable}


% Variable importance: Goodman-standardised coefficients
The relative contribution of each input variable to the overall SICR-prediction $p_1(\boldsymbol{x}_{it})$  can be quantified using an appropriate measure of variable importance. One such classical measure is that of a \textit{Goodman-standardised coefficient} $\beta^*_\mathrm{G}$, whereby a coefficient estimate $\beta$ within a logistic regression model is simply divided by its standard error $SE(\beta)$; see \citet{menard2004six} and \citet{menard2011standards}. 
%By definition, this $\beta^*_\mathrm{G}$-value also equals the $z$-score of the well-known Wald-statistic, which is typically used when testing the statistical significance of an input variable within logistic regression. 
More importantly, one can rank-order the resulting $\beta^*_\mathrm{G}$-values that are associated with the input variables, thereby producing at least a rudimentary ordering of the relative strength (and hence importance) of each input in predicting the outcome. While it would be excessive to provide such an ordering for each of the 27 different SICR-models, we refer the interested reader to our R-codebase on GitHub from \citet{botha2024sourcecode}, which contains some of these orderings. Accordingly, we shall restrict our subsequent analysis to definitions 1a(i)-(iv) in finding commonalities amongst the ranks of $\beta^*_\mathrm{G}$-values within each SICR-model, thereby offering ancillary insight on general patterns of variable importance.


% Variable importance results
% g_0-delinq and its role as the "backstop"
The variable that consistently retained the largest $\beta^*_\mathrm{G}$-value (and hence greatest importance) across all SICR-models is \verb|g0_Delinq|, which is sensible given its typical prominence in PD-models. Moreover, its presence within a SICR-model directly embeds the `backstop' from \S5.5.11 in IFRS 9 since an increase in the $g_0$-measure already constitutes a SICR-event. In this case, the odds ratio also increases substantially by about 900\% on average, which would correctly trigger a SICR-decision across all chosen cut-offs $c_{dsk}$.
% RollEver_24
The second-most important variable 
for SICR-prediction is \verb|RollEver_24|, where a unit increase (i.e., more historical episodes of past delinquency) sensibly increased the odds ratio by 70\% on average.
% ArrearsDir_3 (milling + increasing)
Considering its milling-bin, the variable \verb|ArrearsDir_3| is commonly ranked third, where a constant arrears-level (i.e., maintaining zero arrears) decreased the odds ratio by 60\% on average, relative to the baseline.
Conversely, this variable's increasing-bin fluctuates in its rank from fourth to eight, though all of the aforementioned variables remain delinquency-themed; an interesting result in its own right.
% PayMethod (payroll)
The payroll/cash-bin of the \verb|PayMethod| variable is commonly ranked fourth, where a simple switch in payment method inflated the odds ratio by 78\% on average, which has a similar effect within the PD-model in \cref{app:PD_Model}.
% Prelim_Pc
With its average rank of five, the variable \verb|Prepaid_Pc| measures an aspect of credit capacity in that a 10\%-point improvement therein resulted in a 30\% reduction in the odds ratio on average.
% InterestRate_Margin
Lastly, the sixth-ranked variable \verb|InterestRate_Margin| embeds risk-based pricing information as assessed at loan origination, such that the odds ratio sensibly increased by 17.5\% on average for every 1\%-point increase in the loan price.


